YFS Resummation for Future Lepton-Lepton Colliders in SHERPA

We present an implementation of the Yennie--\-Frautschi--\-Suura (YFS) scheme for the all-orders resummation of logarithms from the emission of soft real and virtual photons in processes that are critical for future lepton colliders. They include, in particular, $e^-e^+\to f\bar{f}$ and $e^-e^+\to W^-W^+$, where we validate the results of our implementation, improved with fixed-order corrections, with those obtained from the most precise calculations. We also show, for the first time, results for the Higgs-Strahlungs process, $e^-e^+\to ZH$, in YFS resummation including fixed-order improvements up to order $\alpha^3L^3$.

==> fsr.tex <==
\subsection{Final State Radiation}\label{SSec::FSR_theory}
In this section, we present an algorithm for generating final state QED radiation
which was developed by Jadach et al in
\cite{Jadach:1999vf}. The algorithm focuses on the emission of
final state soft photons in $\ee \rightarrow f\bar{f},\, f\neq e$, however
this can be extended to calculate FSR for other process such as Higgsstrahlung.
 The calculation is preformed in a reference frame $X$,
 defined by $X = (\sqrt{s}_x,0,0,0)$, where $s_x = (p_1+p_2-\sum_{i}k_i)^2$,
 $p_{1,2}$ are the initial state four-momentum for the case of \eeffbar
 and $k_i$ are the soft photons emitted
 from the initial state. For cases in which there
 are more than two final state particles $s_x$ is constructed from the decaying parent of the dipole $V\rightarrow\ell\bar{\ell}$.
 As the FSR is performed after the ISR in \Sherpa the effect of ISR photons is automatically included.
Let us consider the FSR part of~\Cref{eq:masterYFS}

\begin{equation}\label{Eq:FSRMaster}
  \mathcal{F}_{\bar{n}} = \frac{1}{\bar{n}!} \int_{4m_{f}^2}^{s_x} ds_Q\, \prod_{i=1}^{\bar{n}}
  \int \frac{d^3\bar{k}_i}{\bar{k}^0_i} \tilde{S}_f(\bar{k}_i)\Theta(\bar{k}_i-E_{\text{min}})
  \delta\left(s_X - \left(Q+\sum_{j=0}^{\bar{n}}\bar{k}_j\right)^2\right)e^{Y(q_1,q_2)}
\end{equation}

where $\bar{k}_i$ are the final state soft photons which are defined in the rest frame of the
outgoing dipole momentum $Q=q_1+q_2$. $E_{\text{min}}$ is the energy cut off for the final state photons. Again, we use
an explicit polar parametrization for the photon momentum and with this we can eliminate the
Dirac delta function.
\bea
  \int_{4m_{f}^2}^{s_x} ds_Q\, \delta\left(s_X - \left(Q+\sum_{j=0}^{\bar{n}}\bar{k}_j\right)^2\right) &=&
  \int_{4m_{f}^2}^{s_x} ds_Q\, \delta\left(s_X - s_Q\left(1+\tilde{K}^0+\frac{1}{4}\tilde{K}^2\right)\right) \nonumber \\
  &=& \frac{\Theta(s_Q - 4m^2_f)}{1 + \tilde{K}^0+\frac{1}{4}\tilde{K}^2},
\eea
where,
\bea
\tilde{K} &=& \sum_{i=0}^{\bar{n}} \tilde{k}_i, \nn\\
\tilde{k}_i &=& x_i(1,\sin\theta_i\cos\phi_i, \sin\theta_i\sin\phi_i,\cos\theta_i).
\eea
This means that $s_Q$ now depends on the photon momentum,
\begin{equation}
  s_Q = \frac{s_X}{1 + \tilde{K}^0+\frac{1}{4}\tilde{K}^2}.
\end{equation}
The eikonal term can be treated the same as in the ISR case with the substitution
$m_e \rightarrow m_f,\, s\rightarrow s_Q$.
\beq
  \int \frac{d^3\bar{k}_i}{\bar{k}^0_i} \tilde{S}_f(\bar{k}_i) =
  \int \frac{\dd{x_i}}{x_i}
  \int \frac{\dd{\phi_i}}{2\pi}
  \int  \dd{(\cos\theta_i)}  g\left(\theta_i\right),
\eeq
\beq
  g(\theta) = Z_iZ_j\frac{2\alpha}{\pi}
 \left(\frac{2(1+\beta_i\beta_j)}{(1-\beta_i\cos\theta)(1+\beta_j\cos\theta)}
 -\frac{1-\beta_i^2}{(1-\beta_i\cos\theta)^2}
            -\frac{1-\beta_j^2}{(1+\beta_j\cos\theta)^2}\right).
\eeq
where $\beta_i = \frac{|\vec{p_i}|}{p_i^0}$. This leads to a partially factorized form of
\Cref{Eq:FSRMaster}.
\begin{equation}\label{Eq:FSRSemiFact}
 \mathcal{F}_n =\frac{1}{\bar{n}!}\prod_{i=1}^{\bar{n}} \int_{\epsilon_f}^{\infty} \frac{dx_i}{x_i}
 \int_0^{2\pi} \frac{d\phi_i}{2\pi}
 \int_{-1}^1 d\cos\theta_i \frac{\alpha}{\pi} g\left(\theta_i\right)
 \frac{\Theta\left(s_Q-4m_f^2\right)}{1 + \tilde{K}^0+\frac{1}{4}\tilde{K}^2}e^{Y_{F}(q_1,q_2)}.
\end{equation}
\Cref{Eq:FSRSemiFact} is not yet in a fully factorised form desirable for a Monte Carlo simulation.
Ideally, we would want~\Cref{Eq:FSRMaster} expressed as a product of $\bar{n}$ independent
integrals for each photon. This is not yet the case for~\Cref{Eq:FSRSemiFact}, as there is an
explicit dependence on the sum of the photon momenta in $s_Q$. Another issue that complicates matters is
the fact that the upper limit can be quite large, for example in the case of a hard FSR
photon, which can be inefficient for MC integration. A solution can be found by introducing a
change of variables,
\bea
  y_{i} &=& \frac{x_i}{1+\sum_j x_j} = \frac{x_i}{1+\tilde{K}^0},
  % 1 + \sum_j x_j &=& 1 + \tilde{K}^0
  % \frac{s_X}{s_Q}\left(1-\frac{K^2}{s_X}\right)
\eea
% \bea
%   y_{j} &=& \frac{x_j}{1-\sum_i x_i},\quad x_j = \frac{y_j}{1-\sum_i y_i}\\
%   1 + \sum_i x_i &=&  \frac{1}{1-\sum_jy_j} = 1 + \tilde{K}^0
%   \frac{s_X}{s_Q}\left(1-\frac{K^2}{s_X}\right)
% \eea
where $K= \frac{\sqrt{s_Q}}{2}\tilde{K}$. This transforms~\Cref{Eq:FSRSemiFact} to our
primary distribution,
\begin{align}\label{Eq:PrimaryFSR}
  \mathcal{F}_n =& \frac{1}{\bar{n}!}\prod_{i=1}^{\bar{n}}
  \int_{\frac{\epsilon_f}{1+\tilde{K}^0}}^1\frac{dy_i}{y_i}
  \int_0^{2\pi}\frac{d\phi_j}{2\pi}
  \int_{-1}^{1} d\cos\theta_i\,\,
  \frac{\alpha}{\pi} g\left(\theta_i\right),\nonumber\\
  &\times \frac{1+\tilde{K}^0}{1 + \tilde{K}^0+\frac{1}{4}\tilde{K}^2}
  \Theta(s_Q-4m_f^2)e^{Y_{F}(q_1,q_2)}.
\end{align}
The new lower limit on the photon energy also depends on the total
photon momentum, which is not ideal. This can be fixed by setting
$\epsilon_f = \delta_f(1+\tilde{K}^0)$ where $\delta_f\ll1$. This substitution
leads to a new minimum energy for the soft photons,
$E_{\text{min}} = \delta_f\frac{\sqrts_Q}{2}(1+\tilde{K}^0)$.
Now we are in a position to introduce some simplifications, as we did in
the ISR case, to make~\Cref{Eq:PrimaryFSR} more suited for MC integration.
\begin{itemize}
 \item To remove any dependence on the photon momentum in $s_Q$ is
        achieved trivially by replacing $s_Q \rightarrow s_X$.
 \item We drop the mass term in $g\left(\theta_i\right)$ for numerical
      stability, which leads to a corrective weight
      $\prod\limits_{i=1}^{\bar{n}} \frac{g(\theta_i)}{\tilde{g}(\theta_i)}$.
 \item $\frac{1+\tilde{K}^0}{1 + \tilde{K}^0+\frac{1}{4}\tilde{K}^2}
      \Theta(s_Q-4m_f^2)\rightarrow 1$. This simplification was
      done to remove a complicated dependence on the photon
      momentum.
  \item  $e^{Y_{F}(q_1,q_2)} \rightarrow e^{\bar{\gamma}\ln(\delta_f)}$
\end{itemize}
With these simplifications we arrive at a FSR differential distribution
that can be generated from uniform random numbers.
\begin{equation}\label{Eq:FsrDifferential}
  \frac{d\mathcal{F}_{\bar{n}}}{\prod_{i=1}^{\bar{n}} dy_i d\cos\theta_i d\phi_i}
  = e^{\bar{\gamma}\ln(\delta_f)}
  \left(\frac{\alpha}{2\pi^2}\right)^{\bar{n}}
  \prod_{i=1}^{\bar{n}}\frac{\Theta(y_i-\delta_f)}{y_i}\tilde{g}
  \left(\theta_i, \frac{m_f^2}{s_X}\right),
\end{equation}
and the corrective weight for this simplified distribution is
given by,
\beq
  w_{\text{FSR}} = e^{\gamma_f\ln(\delta_f(1+\tilde{K}^0))-\bar{\gamma}\ln(\delta_f)}
              \frac{1+\tilde{K}^0}{1 + \tilde{K}^0+\frac{1}{4}\tilde{K}^2}
              \Theta(s_Q-4m_f^2)
              \prod_{i=1}^{\bar{n}}\frac{g(\theta_i)}{\tilde{g}(\theta_i)}.
\eeq

While it is not obvious, it can be shown that the FSR photon multiplicity
is again distributed according to a Poissonian. Summing over all photons and
integrating~\Cref{Eq:FsrDifferential} yields,

\bea
  \sum_{\bar{n}}^{\infty} \mathcal{F}_n &=& \sum_{\bar{n}}^{\infty}\frac{1}{\bar{n}!}\prod_{i=1}^{\bar{n}}
                                          \int_{\delta_f}^1 \frac{dy_i}{y_i}
                                          \int_0^{2\pi} \frac{d\phi_i}{2\pi}
                                          \int_{-1}^{1} d\cos\theta_i
                                          \frac{\alpha}{\pi} \tilde{g}\left(\theta_j\right)
                                          e^{\bar{\gamma}\ln(\delta_f)}\nonumber \\
                                      &=& \sum_{\bar{n}}^{\infty}
                                          e^{\bar{\gamma}\ln(\delta_f)}
                                          \frac{1}{\bar{n}!}\left(\bar{\gamma}\ln
                                          \frac{1}{\delta_f}\right)^{\bar{n}} = 1
\eea
From this it can be seen that the average for the photon multiplicity is
$\langle \bar{n} \rangle = \bar{\gamma}\ln\frac{1}{\delta_f} $. Once
we know the multiplicity for a given event we can distribute the
photon momenta as described in \cite{Jadach:1988gb}.
To correct the final state momentum for photon emission,
we define a frame $Q=\left(\sqrt{s_Q},0,0,0\right)$
and a frame $X=Q-\sum_{i}k_i$. We boost the final
states into the frame $X$, then we preform a random
Euler rotation, and finally we boost-back the fermions
to the frame $X$. The Euler rotations have no special
geometrical meaning, it is just preformed to
erase the fermions direction before we boost-back
to $X$.

\subsection{Infrared Boundary for FSR and ISR}
In our previous discussions we have described how the
multi photon phasespace for initial and final state
emissions is generated. We have already introduced infrared
domains in which the photons may reside. For the ISR
photons the domain $\Omega_I$ is defined by rejecting
all photons with $k^0_I < \hsqrts\epsilon$ and for
FSR the domain is defined by
$k^0_F < \delta_f\left(s_Q+\frac{2\sum k_F}{Q}\frac{\sqrt{s_Q}}{2}\right)$
where $s_Q = Q^2 = (q_1+q_2)^2$. Both of these limits are
defined in the CMS frame of the corresponding dipole.
These two regions need to be combined to avoid
any violation of the IR domains. This can be done by
choosing $\delta_f$ small enough that the FSR domain
lies with the ISR domain. This will also require that
we remove any photon that resides in $\delta\Omega = \Omega_I\setminus \Omega_F$.
This removal process does not come for free. As we
are in essence redefining the IR domain the photon
phasespace integration will have changed and a new
distribution for the MC has to be calculated. The photons
in $\delta\Omega$ are not completely hidden as they are
still present in the FSR weight.
\bea
\lefteqn{\lim_{k_i \rightarrow 0} W_{\text{FSR}} (n, k_1, \cdots, k_i, \cdots, k_n)
          = } \nn \\
          & & W_{\text{FSR}}(n-1,k_1, \cdots, k_{i-1}, k_{i+1}, \cdots, k_n)
          \frac{g(\theta_i,\frac{m_f^2}{s_Q})}{\tilde{g}(\theta_i, \frac{m_f^2}{s})}
\eea
and even the softest photon contributes to $g/\tilde{g}$.
To calculate the effect from the photons in $\delta\Omega$
we evaluate the following integral,
\beq
\int_{\delta\Omega} \frac{d^3 k}{k^0} \eikK
          \frac{g(\theta_i,\frac{m_f^2}{s_Q})}{\tilde{g}(\theta_i, \frac{m_f^2}{s})}
          = 2\alpha Q_f^2 \left( \tilde{B}(\Omega_I;\bar{q}_1,\bar{q}_2)
              - \tilde{B}(\Omega_F;\bar{q}_1,\bar{q}_2)   \right).
\eeq
We have multiplied our FSR weight by a corrective
factor which removes this additional term.
\bea\label{Eq::Hidden_W}
W_{\text{Hidden}}& = &\exp\bigg[-2\alpha Q_F^2
              \left( \tilde{B}(\Omega_I;\bar{q}_1,\bar{q}_2)
              - \tilde{B}(\Omega_F;\bar{q}_1,\bar{q}_2)   \right)
              \nn \\
             & &+2\alpha Q_F^2
              \left( \tilde{B}(\Omega_I;q_1,q_2)
              - \tilde{B}(\Omega_F;q_1,q_2)   \right)\bigg]
\eea
where $q_{1,2}$ are the final state momenta after the photon emission
and $\bar{q}_{1,2}$ are scaled momenta such that
$\bar{q}_i^2=m_i^2\frac{s_Q}{s}$. The second term in the exponential
is used to remove $\tilde{B}(\Omega_F)$ from the original YFS
form factor as $\Omega_I$ now includes $\Omega_F$. For more
detail, see \cite{Jadach:1999vf} where Jadach et al work this
out in great detail.


==> isr.tex <==

\subsection{Initial State Radiation}
 % Here we will derive an algorithm for initial state radiation of soft photons.
 This algorithm was first presented in \cite{Jadach:1988gb} and we have recapitulated
 it here for completeness.
 While we concentrate on \ee initial states,
 this method can be generalized to other massive charged particles.
 We will first simplify the distribution by neglecting
 higher-order $\beta$'s in~\Cref{eq:masterYFS} and later introduce
 a corrective weight to account for this simplification.
 By identifying $\beta_0 = \dd{\sigmaborn}(\hat{s})$, where
 $\sqrt{\hat{s}}$ is the reduced centre of mass energy,
 the total cross section, with respect to the Born phasespace,
   can be expressed as,
 \beq\label{Eq:algorithm:truncated}
  \sigma^{\text{ISR}} = e^{Y(\Omega(\epsilon))}\sum_{n=0}^\infty\frac{1}{n!}
  \int \prod_{i=1}^n\left[
  \frac{\dd[3]{k_i}}{k_i^0}\tilde{S}(p_1,p_2,k_i)\right]
  \dd{\sigmaborn}(\hat{s})
 \eeq
 It also
 includes the integration over the Born phasespace,
 which we do not make explicit here as it is treated
 separately within the MC.
To evaluate this integral we need to rewrite the
 multiphoton phasespace so that
 it is more suitable for Monte Carlo integration.
 Following the procedure detailed in \cite{Jadach:1988gb},
 the simplified cross-section can be written as two integrals,
one where there are zero photon emissions and another for the case
where soft photons have been emitted.
\begin{align}\label{Eq:simpleMaster}
\sigma_{\text{simple}}^{\text{ISR}} &= e^{\frac{\gamma}{4} + Z_iZ_j\frac{\alpha}{\pi}(\frac{\pi^2}{3}-\frac{1}{2})}
                          \left[\int_0^\epsilon \dd{v} \gamma v^{\gamma-1} \dd{\sigmaborn}(s)\right.\nn\\
                          &\left.+ \int_{\epsilon}^{v_{\text{max}}} \dd{v} \dd{\sigmaborn}(s(1-v))
                          \mathcal{J}_0(v)\gammabar v^{\gammabar-1}\epsilon^{\gamma-\gammabar}\right].
\end{align}
where the following change of variable, $v = 1 - \frac{\hat{s}}{s}$, has been introduced.
The lower integration limit $\epsilon$ correspond to the infrared cut-off
on the photon energy, $K_{\text{min}} = \epsilon\hsqrts$. The only condition we require
on this limit is  $\epsilon \ll 1$.
The new terms introduced in~\Cref{Eq:simpleMaster} are defined as,
\bea
 % \mathcal{J}(\bar{K}, v) &=& \frac{1}{2}\left(1 + \frac{1}{\sqrt{1-Av}}\right), \quad
 % A = \frac{\bar{K}^2P^2}{(\bar{K}P)^2}, \quad \bar{K} = \sum_{i=1}^n k_i \\
\mathcal{J}_0(v) &=& \frac{1}{2}\left(1 + \frac{1}{\sqrt{1-v}}\right) \\
 % \lambda_0 &=& v\frac{P^2}{\bar{K}P}\frac{1}{1+\sqrt{1-Av}} \\
\gamma &=& \frac{2\alpha}{\pi}
         \left[\frac{1+\beta_1\beta_2}{\beta_1+\beta_2}
          \ln\frac{\left(1+\beta_1\right)
          \left(1+\beta_2\right)}{\left(1-\beta_1\right)
          \left(1-\beta_2\right)}-2\right], \\
\gammabar &=& \frac{2\alpha}{\pi}
         \frac{1+\beta_1\beta_2}{\beta_1+\beta_2}
          \ln\frac{\left(1+\beta_1\right)
          \left(1+\beta_2\right)}{\left(1-\beta_1\right)
          \left(1-\beta_2\right)},
\eea
where $\beta_i= \frac{|\vec{p_i}|}{p_i^0}$.
Now that we have a simplified cross section, which is suitable for Monte Carlo integration, we need to correct
for the simplifications we introduced.
\begin{itemize}
  \item The first corrective weight is associated with dropping the mass term in
        the photon Eikonals, \eik{i}. The weight is simply
        $w_1 = \prod\limits_{i=1}^{n}\frac{g(\theta_i)}{\tilde{g}(\theta_i)}$,
        where $g(\theta)$ and $\tilde{g}(\theta)$ are defined in~\Cref{EQ:theory:GW}.
        Respectively these result from the integration of the full eikonal and the
        reduced eikonal, in which terms $\oforder{\frac{m^2}{s}}$ are neglected.
  \item  Setting $A=1$ in Jacobian, $\mathcal{J}(\bar{K}, v)= \frac{1}{2}\left(1 + \frac{1}{\sqrt{1-Av}}\right)$,
          reduces the Jacobian to $\mathcal{J}_0(v)=\frac{1}{2}\left(1 + \frac{1}{\sqrt{1-v}}\right)$ and
        this simplification is corrected by $w_2 = \frac{\mathcal{J}(\bar{K}, v)}{\mathcal{J}_0(v)}$.
        A more detailed description can be found in~\Cref{APPENDIX:ISR_Algorithim}.
  \item The third corrective weight is a veto on the individual photon
        energies and is defined as $w_3 = \prod_{i=1}^{n_R} \theta(k_i^0-K_{\text{min}})$.
  \item The fourth weight is due to neglecting the higher order corrections
        and will be discussed in~\Cref{SS:NLOQED}.
\end{itemize}
\begin{align}\label{EQ:theory:GW}
g(\theta) &= \frac{\alpha}{\pi^2}
\left(\frac{2(1+\beta_1\beta_2)}{(1-\beta_1\cos\theta)(1+\beta_2\cos\theta)}
 -\frac{1-\beta_1^2}{(1-\beta_1\cos\theta)^2}
            -\frac{1-\beta_2^2}{(1+\beta_2\cos\theta)^2}\right),\nn\\
\tilde{g}(\theta) &=
   \frac{\alpha}{\pi^2}\left(\frac{2(1+\beta_1\beta_2)}{(1-\beta_1\cos\theta)(1+\beta_2\cos\theta)}\right).
 \end{align}
% The above weights account for the transition from~\Cref{Eq:algor:newMaster} to~\Cref{Eq:simpleMaster}. They
% are purely associated with the generation and resummation of soft photons. They do not provide any
% information about higher-order corrections. These corrections will be introduced later as a further
% corrective weight.
% The above weights are a result of integrating the eikonal term
To obtain the total cross section from our simplified version we just multiply our
simple distribution by the product of our corrective weights during the Monte Carlo integration.
The corrected cross section is therefore defined as,
\begin{align}\label{EQ::CorrectedISR}
\dd{\sigma^{ISR}} &= \prod_{i=1}^2 w_i \dd{\sigma^{ISR}_{\text{simple}}}\nn \\
                  &= \prod_{i=1}^{n_R} \left[\theta(k_i^0-K_{\text{min}})
                      \frac{g(\theta_i)}{\tilde{g}(\theta_i)}\right]
                       \frac{\mathcal{J}(\bar{K}, v)}{\mathcal{J}_0(v)}
                       \dd{\sigma^{ISR}_{\text{simple}}}
\end{align}
Now all that remains to complete our calculation is to integrate
\Cref{EQ::CorrectedISR} over $v$, which can be preformed by
standard MC methods. Once the main integration variable, $v$, is
known the photons can be explicitly constructed. The number of
photons is given by a Poissonian distribution with an average,
\bea
\bar{n} &= & \int_{E_{min}}^{E_{max}}\frac{d^3k}{k^0}\eikK\nn \\
&=& - \frac{\alpha}{\pi}Z_1Z_2\theta_1\theta_2
  \ln\left(\frac{E_{max}}{E_{min}}\right)
  \left(\frac{1+\beta_1\beta_2}{\beta_1+\beta_2}
  \ln\frac{\left(1+\beta_1\right)
  \left(1+\beta_2\right)}{\left(1-\beta_1\right)
  \left(1-\beta_2\right)}-2\right).
\eea
Then the $n_R$ photon momenta are distributed as
and rescaled as described in~\Cref{APPENDIX:ISR_Algorithim}.
A reference frame is defined as $P=p_1+p_2-\sum_{i}k_i$
and the incoming momenta are then expressed as
$\hat{p}_{1/2} = \left(\frac{\sqrt{\hat{s}}}{2},0,0,\pm \hat{p}_z\right)$,
where,
\bea
\hat{p}_z = \frac{1}{2\sqrt{\hat{s}}}
            \left[
              (\hat{s}-(m_1-m_2)^2)(\hat{s}-(m_1+m_2)^2)
            \right]^{\frac{1}{2}}
\eea
which are rotated in the z-direction and then boosted in P.
The new momenta are  passed to \Sherpa's phasespace
module \Phasic, which constructs the final states
from the reduced initial states according to the structure
of the Feynman diagrams.


==> macros.tex <==
% \usepackage{amsmath}
% \usepackage{amssymb}

% \usepackage{wrapfig}
% \usepackage{xspace}
% % \usepackage[usenames,dvipsnames]{xcolor}
% \usepackage{graphicx}
% \usepackage{setspace}
% \usepackage{threeparttable}
% \usepackage{relsize}
% \usepackage{ifthen}
% \usepackage{lineno}
% \usepackage{enumerate}
% \usepackage{makeidx}
% \usepackage{showidx}
\usepackage[acronym]{glossaries}
% \setlength{\parindent}{0.0in}
% \setlength{\parskip}{0.0in}

%%% Structuring
\newcommand{\Vp}{\ensuremath{\vphantom{\frac{|^|}{|^|}}}}
\newcommand{\LINE}{\underline{\hspace*{13.5cm}\hphantom{t}}\\}
% \newcommand{\comment}[2][]{\noindent\LINE{\bf{#1}: }{#2}\\\LINE}
% \newcommand{\todo}[1]{\textbf{\color{red}#1}}
%\newcommand{\didit}[1]{\textbf{\color{blue}did it (#1)}}
%\newcommand{\checked}[1]{\hfill{\textbf{\color{green}\checkmark(#1)}}}
% \newcommand{\todo}[1]{\fbox{\begin{minipage}{\textwidth}\textbf{#1}\end{minipage}}}
\newcommand{\didit}[1]{\textbf{\underline{#1}}}
\newcommand{\checked}[1]{\hfill{\textbf{\underline{#1}}}}
\newacronym{mc}{MC}{Monte Carlo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Maths macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_maths}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Physics macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_physics}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Section references
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_refs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Experiments / Machines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_collabs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Software names
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_codes}





==> makefile <==

# simple makefile for latex code

FILENAME=main
PDFNAME=yfs_paper
# LATEX=pdflatex
DIFF=diff-1-v3
#  use lualatex for the final version
LATEX=lualatex

main:
	$(LATEX) $(FILENAME).tex
	make bib
	$(LATEX) $(FILENAME).tex
	$(LATEX) $(FILENAME).tex
	mv $(FILENAME).pdf $(PDFNAME).pdf
	# make clean

diffinit:
	latexpand --makeatletter main.tex > review-1-full-v2.tex
	latexdiff master-full.tex review-1-full-v2.tex > ${DIFF}.tex


diff:
	$(LATEX) $(DIFF).tex 
	make bibdiff
	$(LATEX) $(DIFF).tex
	$(LATEX) $(DIFF).tex
	make clean


bibdiff: 
	bibtex $(DIFF)      


bib: 
	bibtex $(FILENAME)      

read:
	nohup okular $(PDFNAME).pdf > /dev/null 2>&1 &                        

fullclean:                      
	rm -fv $(PDFNAME).pdf   
	make clean              

clean:
	rm -fv $(FILENAME).pdf \
	*.log *.aux *.toc *.out *.fdb_* *.gz *.*synctex* *.fls \
	*.bbl *.bcf *.blg \
	*.acn *.acr *.alg *.glg *.glo *.gls *.ist *.glsdefs *.run.xml *.xdy   


==> makefile_ <==
# simple makefile for latex code

FILENAME=main
PDFNAME=yfs_paper
# LATEX=pdflatex
DIFF=diff-1-v3
#  use lualatex for the final version
LATEX=lualatex

main:
	$(LATEX) $(FILENAME).tex
	make bib
	$(LATEX) $(FILENAME).tex
	$(LATEX) $(FILENAME).tex
	mv $(FILENAME).pdf $(PDFNAME).pdf
	make clean

diffinit:
	latexpand --makeatletter main.tex > review-1-full-v2.tex
	latexdiff master-full.tex review-1-full-v2.tex > ${DIFF}.tex


diff:
	$(LATEX) $(DIFF).tex 
	make bibdiff
	$(LATEX) $(DIFF).tex
	$(LATEX) $(DIFF).tex
	make clean


bibdiff: 
	bibtex $(DIFF)      


bib: 
	bibtex $(FILENAME)      

read:
	nohup okular $(PDFNAME).pdf > /dev/null 2>&1 &                        

fullclean:                      
	rm -fv $(PDFNAME).pdf   
	make clean              

clean:
	rm -fv $(FILENAME).pdf \
	*.log *.aux *.toc *.out *.fdb_* *.gz *.*synctex* *.fls \
	*.bbl *.bcf *.blg \
	*.acn *.acr *.alg *.glg *.glo *.gls *.ist *.glsdefs *.run.xml *.xdy   


==> order-table.tex <==
\begin{figure}[h]
\centering
\begin{tabular}{cc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
--- first table, pragmatic second order
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hbox{
\begin{tabular}{cccccc}
& \multicolumn{3}{c}{$\mathcal{O}(\alpha^1)_{\text{Prag}}$}
\\
% \rowcolor{yellow}
\hhline{|-|}
% \cline{1-1}
\multicolumn{1}{|l|}{\cellcolor{yellow}$1$}
 \\ \hhline{*{0}{~}*{2}{-|}}
 % \\ \hhline{--}
% \\\cline{1-2}
 % \hhline{| |-|}
%
\multicolumn{1}{|l}{\cellcolor{yellow}$\alpha$L} &
\multicolumn{1}{l|}{\cellcolor{yellow}$\alpha$}
% \\ \hhline{|-|-|-|}
\\ \cline{3-3}
%
% \rowcolor{white}
\multicolumn{1}{|l}{$\alpha^2$L$^2$}&
\multicolumn{1}{l}{$\alpha^2$L}       &
\multicolumn{1}{l|}{$\alpha^2$}
% \\ \hhline{|-|-|-|-|}
\\ \cline{4 -4}

%
\multicolumn{1}{|l}{$\alpha^3$L$^3$}  &
\multicolumn{1}{l}{$\alpha^3$L$^2$}   &
\multicolumn{1}{l}{$\alpha^3$L}       &
\multicolumn{1}{l|}{$\alpha^3$}
% \\ \hhline{|-|-|-|-|-|}
\\ \cline{5-5}
%
\multicolumn{1}{|l}{$\alpha^4$L$^4$}  &
\multicolumn{1}{l}{$\alpha^4$L$^3$}   &
\multicolumn{1}{l}{$\alpha^4$L$^2$}   &
\multicolumn{1}{l}{$\alpha^4$L$^1$}   &
\multicolumn{1}{l|}{$\alpha^4$}       &
\hbox{\quad}
% \\ \hhline{|-|-|-|-|-|-|}
\\ \cline{6-6}
\multicolumn{1}{|c}{\vdots} &
\multicolumn{1}{c}{\vdots} &
\multicolumn{1}{c}{\vdots}
%\\
%& \multicolumn{3}{c}{\large (a)}
\end{tabular}}
\quad
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% --- second table, pragmatic third order
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hbox{
\begin{tabular}{llllll}
& \multicolumn{3}{c}{$\mathcal{O}(\alpha^2)_{\text{Prag}}$}
\\
% \rowcolor{yellow}
\hhline{|-|}
% \cline{1-1}
\multicolumn{1}{|l|}{\cellcolor{yellow}$1$}
% \\  \hhline{*{0}{|~|}*{2}{-|}}
\\ \cline{2-2}
%
\multicolumn{1}{|l}{\cellcolor{yellow}$\alpha$L} &
\multicolumn{1}{l|}{\cellcolor{yellow}$\alpha$}
% \\ \hhline{|-|-|-|}
\\ \cline{3-3}
%
% \rowcolor{white}
\multicolumn{1}{|l}{\cellcolor{yellow}$\alpha^2$L$^2$} &
\multicolumn{1}{l}{$\alpha^2$L}       &
\multicolumn{1}{l|}{$\alpha^2$}
% \\ \hhline{|-|-|-|-|}
\\ \cline{4 -4}

%
\multicolumn{1}{|l}{$\alpha^3$L$^3$}  &
\multicolumn{1}{l}{$\alpha^3$L$^2$}   &
\multicolumn{1}{l}{$\alpha^3$L}       &
\multicolumn{1}{l|}{$\alpha^3$}
% \\ \hhline{|-|-|-|-|-|}
\\ \cline{5-5}
%
\multicolumn{1}{|l}{$\alpha^4$L$^4$}  &
\multicolumn{1}{l}{$\alpha^4$L$^3$}   &
\multicolumn{1}{l}{$\alpha^4$L$^2$}   &
\multicolumn{1}{l}{$\alpha^4$L$^1$}   &
\multicolumn{1}{l|}{$\alpha^4$}       &
\hbox{\quad}
% \\ \hhline{|-|-|-|-|-|-|}
\\ \cline{6-6}
\multicolumn{1}{|c}{\vdots} &
\multicolumn{1}{c}{\vdots} &
\multicolumn{1}{c}{\vdots}
%\\
%& \multicolumn{3}{c}{\large (a)}
\end{tabular}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% --- second table, pragmatic third order
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
\hbox{
\begin{tabular}{llllll}
& \multicolumn{3}{c}{\newline$\mathcal{O}(\alpha^3)_{\text{Prag}}$}
\\
% \rowcolor{yellow}
\hhline{|-|}
% \cline{1-1}
\multicolumn{1}{|l|}{\cellcolor{yellow}$1$}
% \\  \hhline{*{0}{|~|}*{2}{-|}}
\\ \cline{2-2}
%
\multicolumn{1}{|l}{\cellcolor{yellow}$\alpha$L} &
\multicolumn{1}{l|}{\cellcolor{yellow}$\alpha$}
% \\ \hhline{|-|-|-|}
\\ \cline{3-3}
%
% \rowcolor{white}
\multicolumn{1}{|l}{\cellcolor{yellow}$\alpha^2$L$^2$} &
\multicolumn{1}{l}{\cellcolor{yellow}$\alpha^2$L}       &
\multicolumn{1}{l|}{$\alpha^2$}
% \\ \hhline{|-|-|-|-|}
\\ \cline{4 -4}

%
\multicolumn{1}{|l}{\cellcolor{yellow}$\alpha^3$L$^3$}  &
\multicolumn{1}{l}{$\alpha^3$L$^2$}   &
\multicolumn{1}{l}{$\alpha^3$L}       &
\multicolumn{1}{l|}{$\alpha^3$}
% \\ \hhline{|-|-|-|-|-|}
\\ \cline{5-5}
%
\multicolumn{1}{|l}{$\alpha^4$L$^4$}  &
\multicolumn{1}{l}{$\alpha^4$L$^3$}   &
\multicolumn{1}{l}{$\alpha^4$L$^2$}   &
\multicolumn{1}{l}{$\alpha^4$L$^1$}   &
\multicolumn{1}{l|}{$\alpha^4$}       &
\hbox{\quad}
% \\ \hhline{|-|-|-|-|-|-|}
\\ \cline{6-6}
\multicolumn{1}{|c}{\vdots} &
\multicolumn{1}{c}{\vdots} &
\multicolumn{1}{c}{\vdots}
%\\
%& \multicolumn{3}{c}{\large (a)}
\end{tabular}}
\end{tabular}
\caption{Contributions to the leading and sub-leading QED corrections.
         The first column is the leading logarithmic (LL)
         contribution, the second column is the next-to-leading
         (NLL) and so on. We have highlighted the
         terms that contribute to our pragmatic
         expansion.}
\label{tab:pragma2}
\end{figure}

==> semi.tex <==
In this chapter we will present numerical results from
the YFS implementation in \Sherpa. First, we shall compare
the total cross section from \Sherpa with the
results of a separate semi-analytical calculation
of~\Cref{eq:masterYFS}.
Secondly, we will present a comparison
with an existing MC tool,
\kkmc\cite{Jadach:1988gb,Jadach:1999vf}, in which YFS
resummation has been implemented.
Predictions of total cross sections are compared
with experimental results from \lep.
We will also discuss the production  WW and ZH  at
energies relevant for future colliders.

\section{Validation}
\subsection{Semi-Analytical Approach}
We shall briefly present the semi-analytical
approach to soft photon resummation and compare the results
from this approach
with our implementation in \Sherpa.
As discussed in \cite{Jadach:2000ir} it can be shown that
\Cref{eq:masterYFS} can be approximated by relatively
simple integrals. This method involves integrating the
entire phasespace analytically as far as possible. This
will then leave one or two dimensional integrals which can be evaluate
using non-MC methods such as numerical quadrature. The non-MC approach was quite popular for
predicting simple observables  at \lep.
For example,
it was used to calculate the cross section for \eeffbar, including ISR and FSR effects, in tools like
TOPAZO\cite{Nicrosini:1986sm} and ZFITTER\cite{Bardin:1999yd}. While the non-MC approach
is far easier to implement than a MC algorithm, it does have significant disadvantages. Generally,
 they are unable to take into account complex experimental cuts as the phasespace is not
 explicitly constructed.
Improving the perturbative accuracy of the semi-analytical approach
is rather complicated, as increasing the multiplicity of the final state makes the analytical integration of
the phasespace difficult, if not impossible. Even with these disadvantages the semi-analytical
approach can provide an accurate prediction of the total cross section at certain orders.
It is therefore a useful independent validation of the MC algorithm.

For ISR, the semi-analytical formula can be written as,
\beq\label{equation:results:semi}
  \sigma = \int_{v_{\text{min}}}^{v_{\text{max}}} \dd{v}\left[ e^{\frac{\gamma}{4}+\gamma_{\text{Euler}}
  + \frac{\alpha}{\pi}\left(-\frac{1}{2} + \frac{\pi^2}{3}\right)}
  \frac{\gamma v^{\gamma-1}}{\Gamma(1+\gamma)}
  d\sigma_{\text{Born}}(s(1-v))
  \left[\mathcal{S}+\mathcal{H}\left(v\right)\right]\right]
\eeq
where $\gamma = \frac{2\alpha}{\pi}\left(\log\frac{s}{m_f^2}-1\right)$, $m_f$ is the mass of
the initial state lepton, $\Gamma$ is the gamma function and $\gamma_{\text{Euler}}$
is the Euler-Mascheroni constant. The expressions for
 $\mathcal{S}\text{ and }  \mathcal{H}(v)$ are given in~\Cref{table:results:semi}.
$d\sigma_{\text{Born}}$ is the spin-averaged differential Born level cross section for \eeffbar,
which is also integrated over the scattering angle $\theta$.
We implemented a non-MC calculation of~\Cref{equation:results:semi} in
a simple Python program, where the integral was evaluated using adaptive
 quadrature methods from the SciPy library\cite{2020SciPy-NMeth}. The total cross section
was calculated at various different $v_{\text{max}}$, a trivial cut that can
be applied in the non-MC approach, and was compared against predictions from
\Sherpa. The input parameters used for both calculations are given in~\Cref{tab:Validation:ew-inputs}.

The lower integration limit, $v_{\text{min}}$, was set to $10^{-5}$. The reduction of $v_{\text{max}}$
was truncated at 0.1 as lower values caused numerical instabilities in
the python implementation.
\begin{figure}
 \begin{center}
    \includegraphics[width=0.8\textwidth]{plots/semi-analytical/semi_compare.pdf}
 \end{center}
 \caption{ Plot of the deviation of the \Sherpa cross section from
          the semi-analytical calculated according to~\Cref{equation:results:semi}
          with increasing cuts on $v$.}
  \label{PLOT::results::semialpha1}
\end{figure}
\begin{table}
\setlength{\tabcolsep}{11pt}
\renewcommand{\arraystretch}{1.5}
\centering
%%%----------------- initial state -------------------------
\def\mystrut{\rule{0pt}{5mm}}
\begin{tabular}{ c||c | c}
% \hline
\mystrut
   % &
      & $\mathcal{S}$
         & $\mathcal{H}(v)$
\\
\hline
$\mathcal{O}(\alpha^0)_{\text{Prag}}$ \mystrut
   % & $\bbeta_0$
      &  $1 $
         & $ -{1\over 4}\gamma\ln\left(1-v\right)
             -{1\over 2} {\alpha\over\pi} \ln^2\left(1-v\right) $
\\
\hline
$\mathcal{O}(\alpha^1)_{\text{Prag}}$ \mystrut
   % & All
      &  $1+{\gamma\over 2} $
         & $v\left(-1+{v\over 2}\right)
              +\gamma\left[
                  -{v^2\over 2} -{\left(1-v\right)^2\over 4}\ln\left(1-v\right)
                    \right]$
\\
\hline
$\mathcal{O}(\alpha^2)_{\text{Prag}}$ \mystrut
   % & All
      &  $1+{\gamma\over 2}+{\gamma^2\over 8} $
         & $v\left(-1+{v\over 2}\right)
              +\gamma\left[
                  -{v\over 2} -{1+3\left(1-v\right)^2\over 4}\ln\left(1-v\right)
                    \right]$
\\
\hline
\end{tabular}
\caption{
  Contributions to the functions $\mathcal{S}$ and $\mathcal{H}\left(v\right)$
  for the semi-analytical approach in~\Cref{equation:results:semi}.
}
\label{table:results:semi}
\end{table}
The deviation between \Sherpa's cross section and the semi-analytical result
is given in~\Cref{PLOT::results::semialpha1}. As we can see in the figure
there is an excellent agreement for all orders. The deviation between the
two implementation is at the 0.1\% level. This results, gives us confidence
that our prediction for the total cross section is correct. However,
it tells us nothing about the differential distributions that are
fully generated in \Sherpa. In the next section we investigate and
validate the full MC approach against existing implementation in \kkmc.

